Tiresias: A Benchmark and Agent for Language-Guided Planning with World Models

World models enable planning through internal simulation, while natural language provides intuitive task specification. Yet, language-conditioned world modeling remains fragmented across domains with disparate action spaces, datasets, and evaluation protocols. We present Tiresias, a framework towards language-guided planning with world models that comprises a shared task, a benchmark, and a reference agent. The task, language-conditioned world modeling, maps an initial agent-view observation and a language instruction to an action sequence that fulfills the instruction. The benchmark, Tiresias-Bench, integrates 15 datasets across navigation, robotics, 3D gaming, and driving under a shared action interface and evaluation protocol, pairing 142,987 episodes with 428,961 instructions in three styles. The agent, Tiresias-Agent, plans via selective imagination: a language-conditioned diffusion policy proposes candidate trajectories, a trajectory ranker shortlists them, a video-pretrained world model imagines the visual consequences of the shortlist, and a visual ranker scores these rollouts; trajectory and visual scores jointly select the final plan. On Tiresias-Bench, Tiresias-Agent attains overall scores of 63 and 51 on the seen and unseen validation splits, improving over the strongest baseline by 9 points on each. Together, Tiresias-Bench and Tiresias-Agent provide a unified evaluation setting and a strong starting point for language-guided planning with world models.

==> sec/0_abstract.tex <==
\begin{abstract}
World models enable planning through internal simulation, while natural language provides intuitive task specification. Yet, language-conditioned world modeling remains fragmented across domains with disparate action spaces, datasets, and evaluation protocols. We present Tiresias, a framework towards language-guided planning with world models that comprises a shared task, a benchmark, and a reference agent. The task, language-conditioned world modeling, maps an initial agent-view observation and a language instruction to an action sequence that fulfills the instruction. The benchmark, \bench{}, integrates 15 datasets across navigation, robotics, 3D gaming, and driving under a shared action interface and evaluation protocol, pairing 142{,}987 episodes with 428{,}961 instructions in three styles. The agent, Tiresias-Agent, plans via selective imagination: a language-conditioned diffusion policy proposes candidate trajectories, a trajectory ranker shortlists them, a video-pretrained world model imagines the visual consequences of the shortlist, and a visual ranker scores these rollouts; trajectory and visual scores jointly select the final plan. On \bench{}, Tiresias-Agent attains overall scores of 63 and 51 on the seen and unseen validation splits, improving over the strongest baseline by 9 points on each. Together, \bench{} and Tiresias-Agent provide a unified evaluation setting and a strong starting point for language-guided planning with world models.
\end{abstract}
